Findings of the First Workshop on Simulating Conversational Intelligence in Chat

The aim of the workshop was to bring together experts working on open-domain dialogue research. In this speedily advancing research area many challenges still exist, such as learning information from conversations, and engaging in a realistic and convincing simulation of human intelligence and reasoning. SCI-CHAT follows previous workshops on open domain dialogue but in contrast the focus of the shared task is simulation of intelligent conversation as judged in a live human evaluation. Models aim to include the ability to follow a challenging topic over a multi-turn conversation, while positing, refuting and reasoning over arguments. The workshop included both a research track and shared task. The main goal of this paper is to provide an overview of the shared task, and an in depth analysis of the shared task results following presentation at the workshop. The current paper is an extension of that made available prior to presentation of results at the workshop at EACL Malta (Graham et al., 2024). The data collected in the evaluation was made publicly available to aide future research. The code was also made available for the same purpose.

==> app-00-topten.tex <==
\appendix
\label{app:topten}

\begin{figure*}[ht]
     \centering
     \input{fig-00-rater-agree}
        \caption{Score Distributions Top 10 Individual Workers}
        \label{fig:topten}
\end{figure*}

==> custom-backup.tex <==
% Use this file for citations not found in the ACL Anthology (contained in "anthology.bib").

@inproceedings{graham-etal-2024-findings,
    title = "Findings of the First Workshop on Simulating Conversational Intelligence in Chat",
    author = "Graham, Yvette  and
      Qureshi, Mohammed Rameez  and
      Khalid, Haider  and
      Lampouras, Gerasimos  and
      Iacobacci, Ignacio  and
      Liu, Qun",
    editor = "Graham, Yvette  and
      Liu, Qun  and
      Lampouras, Gerasimos  and
      Iacobacci, Ignacio  and
      Madden, Sinead  and
      Khalid, Haider  and
      Qureshi, Rameez",
    booktitle = "Proceedings of the 1st Workshop on Simulating Conversational Intelligence in Chat (SCI-CHAT 2024)",
    month = mar,
    year = "2024",
    address = "St. Julians, Malta",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2024.scichat-1.1",
    pages = "1--3",
    abstract = "The aim of this workshop is to bring together experts working on open-domain dialogue research. In this speedily advancing research area many challenges still exist, such as learning information from conversations, engaging in realistic and convincing simulation of human intelligence and reasoning. SCI-CHAT follows previous workshops on open domain dialogue but with a focus on the simulation of intelligent conversation as judged in a live human evaluation. Models aim to include the ability to follow a challenging topic over a multi-turn conversation, while positing, refuting and reasoning over arguments. The workshop included both a research track and shared task. The main goal of this paper is to provide an overview of the shared task and a link to an additional paper that will include an in depth analysis of the shared task results following presentation at the workshop.",
}

@misc{awad2023overview,
      title={An overview on the evaluated video retrieval tasks at TRECVID 2022}, 
      author={George Awad and Keith Curtis and Asad Butt and Jonathan Fiscus and Afzal Godil and Yooyoung Lee and Andrew Delgado and Eliot Godard and Lukas Diduch and Jeffrey Liu and Yvette Graham and Georges Quenot},
      year={2023},
      eprint={2306.13118},
      archivePrefix={arXiv},
      primaryClass={cs.AI}
}



@inproceedings{graham-etal-2020-assessing,
    title = "Assessing Human-Parity in Machine Translation on the Segment Level",
    author = "Graham, Yvette  and
      Federmann, Christian  and
      Eskevich, Maria  and
      Haddow, Barry",
    editor = "Cohn, Trevor  and
      He, Yulan  and
      Liu, Yang",
    booktitle = "Findings of the Association for Computational Linguistics: EMNLP 2020",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.findings-emnlp.375",
    doi = "10.18653/v1/2020.findings-emnlp.375",
    pages = "4199--4207",
    abstract = "Recent machine translation shared tasks have shown top-performing systems to tie or in some cases even outperform human translation. Such conclusions about system and human performance are, however, based on estimates aggregated from scores collected over large test sets of translations and unfortunately leave some remaining questions unanswered. For instance, simply because a system significantly outperforms the human translator on average may not necessarily mean that it has done so for every translation in the test set. Firstly, are there remaining source segments present in evaluation test sets that cause significant challenges for top-performing systems and can such challenging segments go unnoticed due to the opacity of current human evaluation procedures? To provide insight into these issues we carefully inspect the outputs of top-performing systems in the most recent WMT-19 news translation shared task for all language pairs in which a system either tied or outperformed human translation. Our analysis provides a new method of identifying the remaining segments for which either machine or human perform poorly. For example, in our close inspection of WMT-19 English to German and German to English we discover the segments that disjointly proved a challenge for human and machine. For English to Russian, there were no segments included in our sample of translations that caused a significant challenge for the human translator, while we again identify the set of segments that caused issues for the top-performing system.",
}

@inproceedings{mille-etal-2020-third,
    title = "The Third Multilingual Surface Realisation Shared Task ({SR}{'}20): Overview and Evaluation Results",
    author = "Mille, Simon  and
      Belz, Anya  and
      Bohnet, Bernd  and
      Castro Ferreira, Thiago  and
      Graham, Yvette  and
      Wanner, Leo",
    editor = "Belz, Anya  and
      Bohnet, Bernd  and
      Ferreira, Thiago Castro  and
      Graham, Yvette  and
      Mille, Simon  and
      Wanner, Leo",
    booktitle = "Proceedings of the Third Workshop on Multilingual Surface Realisation",
    month = dec,
    year = "2020",
    address = "Barcelona, Spain (Online)",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.msr-1.1",
    pages = "1--20",
    abstract = "This paper presents results from the Third Shared Task on Multilingual Surface Realisation (SR{'}20) which was organised as part of the COLING{'}20 Workshop on Multilingual Surface Realisation. As in SR{'}18 and SR{'}19, the shared task comprised two tracks: (1) a Shallow Track where the inputs were full UD structures with word order information removed and tokens lemmatised; and (2) a Deep Track where additionally, functional words and morphological information were removed. Moreover, each track had two subtracks: (a) restricted-resource, where only the data provided or approved as part of a track could be used for training models, and (b) open-resource, where any data could be used. The Shallow Track was offered in 11 languages, whereas the Deep Track in 3 ones. Systems were evaluated using both automatic metrics and direct assessment by human evaluators in terms of Readability and Meaning Similarity to reference outputs. We present the evaluation results, along with descriptions of the SR{'}19 tracks, data and evaluation methods, as well as brief summaries of the participating systems. For full descriptions of the participating systems, please see the separate system reports elsewhere in this volume.",
}

@inproceedings{mille-etal-2019-second,
    title = "The Second Multilingual Surface Realisation Shared Task ({SR}{'}19): Overview and Evaluation Results",
    author = "Mille, Simon  and
      Belz, Anja  and
      Bohnet, Bernd  and
      Graham, Yvette  and
      Wanner, Leo",
    editor = "Mille, Simon  and
      Belz, Anja  and
      Bohnet, Bernd  and
      Graham, Yvette  and
      Wanner, Leo",
    booktitle = "Proceedings of the 2nd Workshop on Multilingual Surface Realisation (MSR 2019)",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D19-6301",
    doi = "10.18653/v1/D19-6301",
    pages = "1--17",
    abstract = "We report results from the SR{'}19 Shared Task, the second edition of a multilingual surface realisation task organised as part of the EMNLP{'}19 Workshop on Multilingual Surface Realisation. As in SR{'}18, the shared task comprised two tracks with different levels of complexity: (a) a shallow track where the inputs were full UD structures with word order information removed and tokens lemmatised; and (b) a deep track where additionally, functional words and morphological information were removed. The shallow track was offered in eleven, and the deep track in three languages. Systems were evaluated (a) automatically, using a range of intrinsic metrics, and (b) by human judges in terms of readability and meaning similarity. This report presents the evaluation results, along with descriptions of the SR{'}19 tracks, data and evaluation methods. For full descriptions of the participating systems, please see the separate system reports elsewhere in this volume.",
}

@inproceedings{mille-etal-2018-first,
    title = "The First Multilingual Surface Realisation Shared Task ({SR}{'}18): Overview and Evaluation Results",
    author = "Mille, Simon  and
      Belz, Anja  and
      Bohnet, Bernd  and
      Graham, Yvette  and
      Pitler, Emily  and
      Wanner, Leo",
    editor = "Mille, Simon  and
      Belz, Anja  and
      Bohnet, Bernd  and
      Pitler, Emily  and
      Wanner, Leo",
    booktitle = "Proceedings of the First Workshop on Multilingual Surface Realisation",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W18-3601",
    doi = "10.18653/v1/W18-3601",
    pages = "1--12",
    abstract = "We report results from the SR{'}18 Shared Task, a new multilingual surface realisation task organised as part of the ACL{'}18 Workshop on Multilingual Surface Realisation. As in its English-only predecessor task SR{'}11, the shared task comprised two tracks with different levels of complexity: (a) a shallow track where the inputs were full UD structures with word order information removed and tokens lemmatised; and (b) a deep track where additionally, functional words and morphological information were removed. The shallow track was offered in ten, and the deep track in three languages. Systems were evaluated (a) automatically, using a range of intrinsic metrics, and (b) by human judges in terms of readability and meaning similarity. This report presents the evaluation results, along with descriptions of the SR{'}18 tracks, data and evaluation methods. For full descriptions of the participating systems, please see the separate system reports elsewhere in this volume.",
}

@inproceedings{graham-etal-2017-improving,
    title = "Improving Evaluation of Document-level Machine Translation Quality Estimation",
    author = "Graham, Yvette  and
      Ma, Qingsong  and
      Baldwin, Timothy  and
      Liu, Qun  and
      Parra, Carla  and
      Scarton, Carolina",
    editor = "Lapata, Mirella  and
      Blunsom, Phil  and
      Koller, Alexander",
    booktitle = "Proceedings of the 15th Conference of the {E}uropean Chapter of the Association for Computational Linguistics: Volume 2, Short Papers",
    month = apr,
    year = "2017",
    address = "Valencia, Spain",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/E17-2057",
    pages = "356--361",
    abstract = "Meaningful conclusions about the relative performance of NLP systems are only possible if the gold standard employed in a given evaluation is both valid and reliable. In this paper, we explore the validity of human annotations currently employed in the evaluation of document-level quality estimation for machine translation (MT). We demonstrate the degree to which MT system rankings are dependent on weights employed in the construction of the gold standard, before proposing direct human assessment as a valid alternative. Experiments show direct assessment (DA) scores for documents to be highly reliable, achieving a correlation of above 0.9 in a self-replication experiment, in addition to a substantial estimated cost reduction through quality controlled crowd-sourcing. The original gold standard based on post-edits incurs a 10{--}20 times greater cost than DA.",
}

@inproceedings{ma-etal-2017-investigation,
    title = "Further Investigation into Reference Bias in Monolingual Evaluation of Machine Translation",
    author = "Ma, Qingsong  and
      Graham, Yvette  and
      Baldwin, Timothy  and
      Liu, Qun",
    editor = "Palmer, Martha  and
      Hwa, Rebecca  and
      Riedel, Sebastian",
    booktitle = "Proceedings of the 2017 Conference on Empirical Methods in Natural Language Processing",
    month = sep,
    year = "2017",
    address = "Copenhagen, Denmark",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D17-1262",
    doi = "10.18653/v1/D17-1262",
    pages = "2476--2485",
    abstract = "Monolingual evaluation of Machine Translation (MT) aims to simplify human assessment by requiring assessors to compare the meaning of the MT output with a reference translation, opening up the task to a much larger pool of genuinely qualified evaluators. Monolingual evaluation runs the risk, however, of bias in favour of MT systems that happen to produce translations superficially similar to the reference and, consistent with this intuition, previous investigations have concluded monolingual assessment to be strongly biased in this respect. On re-examination of past analyses, we identify a series of potential analytical errors that force some important questions to be raised about the reliability of past conclusions, however. We subsequently carry out further investigation into reference bias via direct human assessment of MT adequacy via quality controlled crowd-sourcing. Contrary to both intuition and past conclusions, results for show no significant evidence of reference bias in monolingual evaluation of MT.",
}

@inproceedings{kocmi-etal-2022-findings,
    title = "Findings of the 2022 Conference on Machine Translation ({WMT}22)",
    author = "Kocmi, Tom  and
      Bawden, Rachel  and
      Bojar, Ond{\v{r}}ej  and
      Dvorkovich, Anton  and
      Federmann, Christian  and
      Fishel, Mark  and
      Gowda, Thamme  and
      Graham, Yvette  and
      Grundkiewicz, Roman  and
      Haddow, Barry  and
      Knowles, Rebecca  and
      Koehn, Philipp  and
      Monz, Christof  and
      Morishita, Makoto  and
      Nagata, Masaaki  and
      Nakazawa, Toshiaki  and
      Nov{\'a}k, Michal  and
      Popel, Martin  and
      Popovi{\'c}, Maja",
    editor = {Koehn, Philipp  and
      Barrault, Lo{\"\i}c  and
      Bojar, Ond{\v{r}}ej  and
      Bougares, Fethi  and
      Chatterjee, Rajen  and
      Costa-juss{\`a}, Marta R.  and
      Federmann, Christian  and
      Fishel, Mark  and
      Fraser, Alexander  and
      Freitag, Markus  and
      Graham, Yvette  and
      Grundkiewicz, Roman  and
      Guzman, Paco  and
      Haddow, Barry  and
      Huck, Matthias  and
      Jimeno Yepes, Antonio  and
      Kocmi, Tom  and
      Martins, Andr{\'e}  and
      Morishita, Makoto  and
      Monz, Christof  and
      Nagata, Masaaki  and
      Nakazawa, Toshiaki  and
      Negri, Matteo  and
      N{\'e}v{\'e}ol, Aur{\'e}lie  and
      Neves, Mariana  and
      Popel, Martin  and
      Turchi, Marco  and
      Zampieri, Marcos},
    booktitle = "Proceedings of the Seventh Conference on Machine Translation (WMT)",
    month = dec,
    year = "2022",
    address = "Abu Dhabi, United Arab Emirates (Hybrid)",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.wmt-1.1",
    pages = "1--45",
    abstract = "This paper presents the results of the General Machine Translation Task organised as part of the Conference on Machine Translation (WMT) 2022. In the general MT task, participants were asked to build machine translation systems for any of 11 language pairs, to be evaluated on test sets consisting of four different domains. We evaluate system outputs with human annotators using two different techniques: reference-based direct assessment and (DA) and a combination of DA and scalar quality metric (DA+SQM).",
}

@inproceedings{ma-etal-2017-blend,
    title = "{B}lend: a Novel Combined {MT} Metric Based on Direct Assessment {---} {CASICT}-{DCU} submission to {WMT}17 Metrics Task",
    author = "Ma, Qingsong  and
      Graham, Yvette  and
      Wang, Shugen  and
      Liu, Qun",
    editor = "Bojar, Ond{\v{r}}ej  and
      Buck, Christian  and
      Chatterjee, Rajen  and
      Federmann, Christian  and
      Graham, Yvette  and
      Haddow, Barry  and
      Huck, Matthias  and
      Yepes, Antonio Jimeno  and
      Koehn, Philipp  and
      Kreutzer, Julia",
    booktitle = "Proceedings of the Second Conference on Machine Translation",
    month = sep,
    year = "2017",
    address = "Copenhagen, Denmark",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W17-4768",
    doi = "10.18653/v1/W17-4768",
    pages = "598--603",
}

@inproceedings{graham-etal-2016-glitters,
    title = "Is all that Glitters in Machine Translation Quality Estimation really Gold?",
    author = "Graham, Yvette  and
      Baldwin, Timothy  and
      Dowling, Meghan  and
      Eskevich, Maria  and
      Lynn, Teresa  and
      Tounsi, Lamia",
    editor = "Matsumoto, Yuji  and
      Prasad, Rashmi",
    booktitle = "Proceedings of {COLING} 2016, the 26th International Conference on Computational Linguistics: Technical Papers",
    month = dec,
    year = "2016",
    address = "Osaka, Japan",
    publisher = "The COLING 2016 Organizing Committee",
    url = "https://aclanthology.org/C16-1294",
    pages = "3124--3134",
    abstract = "Human-targeted metrics provide a compromise between human evaluation of machine translation, where high inter-annotator agreement is difficult to achieve, and fully automatic metrics, such as BLEU or TER, that lack the validity of human assessment. Human-targeted translation edit rate (HTER) is by far the most widely employed human-targeted metric in machine translation, commonly employed, for example, as a gold standard in evaluation of quality estimation. Original experiments justifying the design of HTER, as opposed to other possible formulations, were limited to a small sample of translations and a single language pair, however, and this motivates our re-evaluation of a range of human-targeted metrics on a substantially larger scale. Results show significantly stronger correlation with human judgment for HBLEU over HTER for two of the nine language pairs we include and no significant difference between correlations achieved by HTER and HBLEU for the remaining language pairs. Finally, we evaluate a range of quality estimation systems employing HTER and direct assessment (DA) of translation adequacy as gold labels, resulting in a divergence in system rankings, and propose employment of DA for future quality estimation evaluations.",
}

@inproceedings{graham-2015-evaluating,
    title = "Re-evaluating Automatic Summarization with {BLEU} and 192 Shades of {ROUGE}",
    author = "Graham, Yvette",
    editor = "M{\`a}rquez, Llu{\'\i}s  and
      Callison-Burch, Chris  and
      Su, Jian",
    booktitle = "Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing",
    month = sep,
    year = "2015",
    address = "Lisbon, Portugal",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D15-1013",
    doi = "10.18653/v1/D15-1013",
    pages = "128--137",
}

@inproceedings{graham-etal-2014-machine,
    title = "Is Machine Translation Getting Better over Time?",
    author = "Graham, Yvette  and
      Baldwin, Timothy  and
      Moffat, Alistair  and
      Zobel, Justin",
    editor = "Wintner, Shuly  and
      Goldwater, Sharon  and
      Riezler, Stefan",
    booktitle = "Proceedings of the 14th Conference of the {E}uropean Chapter of the Association for Computational Linguistics",
    month = apr,
    year = "2014",
    address = "Gothenburg, Sweden",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/E14-1047",
    doi = "10.3115/v1/E14-1047",
    pages = "443--451",
}

@inproceedings{graham-etal-2013-continuous,
    title = "Continuous Measurement Scales in Human Evaluation of Machine Translation",
    author = "Graham, Yvette  and
      Baldwin, Timothy  and
      Moffat, Alistair  and
      Zobel, Justin",
    editor = "Pareja-Lora, Antonio  and
      Liakata, Maria  and
      Dipper, Stefanie",
    booktitle = "Proceedings of the 7th Linguistic Annotation Workshop and Interoperability with Discourse",
    month = aug,
    year = "2013",
    address = "Sofia, Bulgaria",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W13-2305",
    pages = "33--41",
}

@article{convai2paper,
  author    = {Emily Dinan and
               Varvara Logacheva and
               Valentin Malykh and
               Alexander H. Miller and
               Kurt Shuster and
               Jack Urbanek and
               Douwe Kiela and
               Arthur Szlam and
               Iulian Serban and
               Ryan Lowe and
               Shrimai Prabhumoye and
               Alan W. Black and
               Alexander I. Rudnicky and
               Jason Williams and
               Joelle Pineau and
               Mikhail Burtsev and
               Jason Weston},
  title     = {The Second Conversational Intelligence Challenge (ConvAI2)},
  journal   = {CoRR},
  volume    = {abs/1902.00098},
  year      = {2019},
  url       = {http://arxiv.org/abs/1902.00098},
  archivePrefix = {arXiv},
  eprint    = {1902.00098},
  timestamp = {Thu, 30 Jul 2020 17:57:23 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1902-00098.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}





